Quantum Complexity Classes

In our thesis, we try to shed more light onto the complexity of quantum complexity classes by refining the related part of the hierarchy. First, we review the basic concepts of quantum computing in general. Then, inspired by BQP, we define new complexity classes. They are placed between BPP and PSPACE. We show that they incorporate the current important quantum algorithms. Furthermore, the importance of the unitarity constraint given by quantum mechanics is revealed. Without this requirement, we naturally arrive at the class AWPP, which was up to now thought to be just an artificially defined class. We hope that some of our newly defined classes could find their use in proving results about BQP.

==> commands.tex <==
\usepackage{latexsym,amsmath}
\usepackage{amssymb,amsthm}
\pagestyle{headings}

%my commands
\newcommand{\mytitle}[1]{{\huge{#1}}} 

\newcommand{\ou }{\accent23u}
\newcommand{\br}{\begin{eqnarray*}}
\newcommand{\er}{\end{eqnarray*}}
\newcommand{\pk}{\leftrightarrow}
\newcommand{\ro}{\varrho}
\newcommand{\eps}{\epsilon}
\newcommand{\ket}[1]{\arrowvert{#1}\rangle }
\newcommand{\2}{\frac{1}{\sqrt{2}}}

\newcommand{\Ket}[2]{\Big\lgroup \begin{array}{c} #1 \\ #2 \end{array} \Big\rgroup}
\newcommand{\Gate}[4]{\Big\lgroup \begin{array}{rr} #1 & #2 \\ #3 & #4 \end{array} \Big\rgroup}

\newcommand{\BigGate}[4]{\left( \begin{array}{rrrr} #1 \\ #2 \\ #3 \\ #4 \end{array} \right)}
\newcommand{\BigVec}[4]{\left( \begin{array}{r} #1 \\ #2 \\ #3 \\ #4 \end{array} \right)}

\newcommand{\Hadamard}{\frac{1}{\sqrt{2}}\Big\lgroup \begin{array}{rr} 1 & 1 \\ 1 & -1 \end{array} \Big\rgroup}
\newcommand{\CNOT}{\BigGate{1 & 0 & 0 & 0}{0 & 1 & 0 & 0}{0 & 0 & 0 & 1}{0 & 0 & 1 & 0}}

\newcommand{\bra}[1]{\langle{#1}\arrowvert}
\newcommand{\braket}[2]{\langle{#1}\arrowvert{#2}\rangle}
\newcommand{\lit}[1]{[{#1}]}
\newcommand{\up}{\uparrow}
\newcommand{\down}{\downarrow}

\newtheorem{law}{Law}[chapter]
\newtheorem{req}{Requirement}[law]
\newtheorem{lemma}[law]{Lemma}
\newtheorem*{inner}{Nested lemma}
\newtheorem{ex}{Example}[chapter]
\newtheorem{df}{Definition}[chapter]
\newtheorem{cor}[law]{Corollary}
\newtheorem{obs}[law]{Observation}
\newtheorem{theorem}[law]{Theorem}
\newtheorem{hyp}[law]{Hypothesis}

\newcommand{\lref}[1]{law \ref{#1}}
\newcommand{\eqdef}{\overset{\text{\begin{tiny}DEF\end{tiny}}}{=}}

\newcommand{\tl}[1]{\mathbb{#1}}
\newcommand{\CZ}{CZ}
\newcommand{\alfa}{\alpha}
\newcommand{\vk}[1]{\overrightarrow{#1}}
\newcommand{\norm}[1]{\lvert{#1}\rvert}
\newcommand{\bignorm}[1]{\Bigl\lvert{#1}\Bigr\rvert}
\newcommand{\Bignorm}[1]{\Biggl\lvert{#1}\Biggr\rvert}
\newcommand{\TM}{{Turing machine}}
\newcommand{\NTM}{{nondeterministic Turing machine}}
\newcommand{\PTM}{{probabilistic Turing machine}}
\newcommand{\QTM}{{quantum Turing machine}}
\newcommand{\SE}{Schr\"odinger equation}
\newcommand{\her}{^{\dagger}}

\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\sign}{sign}

==> conclusion.tex <==
We summarized the concept of Quantum Computing, both from the view of \QTM s and the view of Quantum circuits.
We also showed the relation between the two models and touched the phenomenon of entanglement.
Then we reviewed some properties of the class $BQP$,  a class of problems that are efficiently solvable by quantum Turing machines and quantum circuits.

In Chapter \ref{nqclasses}, we define a new bunch of classes
inspired by the quantum world and the class $BQP$. Their definitions are natural generalizations or modifications of the definition of $BQP$. One part was obtained by changing the condition
that a circuit be of a polynomial size into the condition that each element of a matrix representing a circuit be a polynomial time computable function and
we may have more identical matrices in the circuit. So we arrived at a bunch of classes $BQ^{t(n)}$ for $t(n)$ being some function that tells us how many
identical matrices in the circuit we have for an input of length $n$. 
This definition is very easy to work with. 
Generalizing this definition to the possibility of more accepting
configurations, we arrived at the family $MQ^{t(n)}$. 
The relation between the classes is that for each $i$: $BQ^i \subseteq MQ^i$. 
All these classes form a huge hierarchy and are all contained in the class $AWPP$.
However, none of the inclusions is known to collapse, nor to be proper. 
Showing a proper inclusion would immediately lead to $P\neq PSPACE$, which is considered to be a very hard question.

From above, it followed that $BQ^{poly(n)}\supseteq BQP$.
 Nevertheless, we showed that the two main quantum algorithms, Deutsch-Jozsza and Shor algorithm belong to the class $BQ^2$ and $MQ^2$ respectively, which raises the question whether the $poly(n)$
in $BQ^{poly(n)}$ can be bounded for example to be a linear function or a constant, or at least
to put $BQP \subseteq MQ^{t(n)}$ with $t(n)$ being something smaller than a general polynomial.

To come back to the classical world, we loosened the definitions of the classes $MQ^{t(n)}$ and $BQ^{t(n)}$ even more and dropped the unitarity condition of the matrices to arrive at the class $M^2$ which is shown to be equal to the class $AWPP$ defined by \cite{pp}. 
This class was invented as an artificial class meant to be used just for proving lowness theorem of $BQP$. 
Here we showed that its definition was surprisingly natural.

The advantage of all these new classes is that they sit in  the hierarchy between $BQP$, $BPP$ and $AWPP$ and are $\Sigma_2$
definable with easy definitions resembling the definition of $BPP$ and $BQP$, and so fill the gap between the wellknown classes
$BQP$ and $AWPP$ in a hierarchy where proving many things is considered to be very hard, such as whether $AWPP=BQP$.
The classes suggested here therefore leave place for future proofs which might lead to showing some properties
of $BQP$ itself. They may also help to understand better how the unitarity of the nature influences computation in general.
\thispagestyle{plain}

==> intro.tex <==
%********************************************************************************************************************
%   INTRO
%********************************************************************************************************************
Quantum computing is concerned with examining how the laws of quantum mechanics can be used to
construct computation devices that would be possibly more powerful than the ''classical ones'', represented by Turing machines.
As was pointed out in \cite{feynman}, computational devices behaving according to the quantum mechanics are not captured
by the classical Church-Turing thesis stating that any practically realizable computational device can be simulated by a Turing machine.
The reason is that the model of \TM s is built implicitly assuming the laws of classical (e.g.\ nonquantum) physics hold, through it may seem that in the model there is no physics involved. 

Thus, if we believe that the quantum theory is correct, we have to generalize the thesis to: ''Any practically realizable computational device
can be simulated by a quantum mechanical device.'' This automatically contains the classical Church-Turing thesis, since huge enough quantum
systems may be described by the laws of classical physics with practically infinite precision. This generalized thesis gave rise to interest in quantum computing. 

This research field entered much into fashion mainly thanks to Peter W. Shor, who published in 1994 his algorithm that can \emph{efficiently} factor
a given number \cite{shor}. Here the word efficiently means in polynomial time with respect to the length of the input.
It's exponentially faster than any other known algorithm for a deterministic Turing machine. 
The problem of finding a factor of a given number is the core of many cryptographic systems, where it is assumed that to factor a large number is practically impossible in a reasonable time. It is believed to be a one-way problem: Multiplying up few numbers is very easy and can be done efficiently, while any known algorithm for a Turing machine requires exponential time.

After the algorithm, nowadays very famous, appeared, there has
been a big rush for other algorithms showing an exponential
speedup over classical algorithms. Surprisingly, until
now, no other quantum algorithm
\footnote{or more precisely an algorithm based on a different idea which is here the quantum Fourier transform}
in the nonrelativized (eg. without
oracles) setting that would offer such a speedup is known.
Furthermore, there is not any physical realization known, that
would allow to build computers with an unbounded amount of
quantum bits without an exponential slowdown. In any case, before any serious
attempt to build a quantum computer the question ''How useful
could a quantum computer be?" must be answered.

The class $BQP$ that contains all problems efficiently computable on a quantum computer should be well understood and placed into to the right place between other well-known traditional complexity classes like \emph{NP}, \emph{BPP}, etc. However nowadays, even fundamental questions like
''Does $BQP$ contain NP-complete problems?" and "Does $BQP$ belong to the polynomial hierarchy?" still remain unanswered.
Nor the lower bounds nor the upper bounds of the complexity of the class $BQP$ are very tight. A possible reason can be that
finding answers to such fundamental questions about the class $BQP$ would immediately answer other fundamental questions from classical complexity theory that are considered to be very hard. For example, showing $BPP\neq BQP$ would immediately imply that $P\neq PSPACE$.
Another reason might be that, through exactly formalized it is, the class $BQP$ is somehow counterintuitive and hard to work with. Intuitively, it would be easier to find relations between two quantum classes than between one conventional and one quantum class. A possible approach to go round these problems and still provide a better insight to the complexity of the class $BQP$ is to define a new bunch of classes somehow inspired by the $BQP$ class, place them to the conventional class hierarchy and then show some interesting properties of them together with their relation to $BQP$. One of such bunches is suggested here.

The aim of this paper is to first review the model of quantum computation, both from the view of Quantum Turing machines and the view of
Quantum circuits. The relation between those two is sketched and also the phenomenon of entanglement and its importance are discussed.
The main work comes after that. We introduce new quantum complexity classes related to the $BQP$ class and show their properties. 

%********************************************************************************************************************
%   ORGANIZATION
%********************************************************************************************************************
This thesis is organized as follows: In chapter \ref{qtm} we
define the \QTM\ and show some of its properties. In the next
chapter, we introduce quantum circuits. Chapter \ref{putting}
shows the relations between quantum circuits and quantum Turing
machines. We focus on comparing the power of the two models. 
The main results of this work show up in chapter \ref{nqclasses}. 
Therein, we define new complexity classes and show some interesting properties of them. 
The new hierarchy of classes is illustrated in section \ref{newclasses}, Figure \ref{newclasses}, together
with some other well-known complexity classes.




==> querymodel.tex <==
\section{Quantum query model}\index{black box model}\index{quantum query model}\index{query model!quantum}
As we let \QTM s access additional information via oracles, we will also allow the circuits to access some kind of additional information.
Here, in the model of quantum circuits, the oracle is picturized as a special type of a gate, called ''black box'' to emphasize we can not see its internal structure. It acts on registers of the form  $\ket{x,b}$ as $$\ket{x,b}\underrightarrow{O}\ket{x,y\oplus I(x)},$$
where $b$ is a single qubit and $I(x)$ is the indicator of $x$. This unit is thus effectively equivalent to the oracle unit used in oracle \QTM s.
As before, we need to assume one more thing comparing to classical black boxes: The quantum black-box needs to support superposition, e.g. to behave as a linear operator.
The black-box model has turned out to be very fruitful for various results, see for example \cite{dj}.

==> requirements.tex <==
In the text, we assume that the reader is familiar with basic linear algebra and
with basic notion of complexity classes and Turing machines. We do not assume any kind of physics knowledge. 
Those, who are interested in the notion of Quantum Computing from a computer scientist point of view, can start from the beginning with chapter \ref{qtm}.  
Those, who are already familiar with Quantum Computing and are only interested in the new bunch of classes, can refer to chapter \ref{nqclasses}.

